Potatoes and Onions

The first major step in the theory of graph minors of Robertson and Seymour was the grid theorem, a fundamental duality result describing that any graph of sufficiently high treewidth must contain a large grid as a minor. Since this pioneering work, multiple grid theorems have been established in structural graph theory, linking various width parameters of combinatorial objects with the non-existence of grid-like obstructions. In particular, Kawarabayashi and Kreutzer [STOC'15] proved a variant of the grid theorem for directed graphs that links directed treewidth with the non-existence of topological minors of large cylindrical walls. On the other hand, to study immersions of undirected graphs $-$ another containment relation that focuses on edge-disjointness, rather than vertex-disjointness $-$ Wollan [JCTB'15] introduced a parameter, tree-cutwidth, and proved that it is dual to immersions of large walls. In this work, we present a version of Wollan's parameter for directed graphs, the directed tree-cutwidth. The main result is a grid theorem for directed tree-cutwidth, establishing that it is dual to directed immersions of large cylindrical walls.

==> app-HS.tex <==
\section{Equivalence of directed treewidth and HS-\cyclewidth}\label{sec:HS}


%\TD{add that HS-cyclewidth is closed under butterfly minors}

In this section we prove the relation between directed treewidth and HS-\cyclewidth.

\dtwHSw*

We split the proof into two lemmas, each proving one of the inequalities.

\begin{lemma}
	\label{lem:dtw_bounds_hsw}
	Let \(D\) be a digraph of directed \treewidth \(w\).
	Then \(D\) has HS-\cyclewidth at most \(w + 1\).
\end{lemma}
\begin{proof}
	Let \((\widehat{T}, \widehat{\beta}, \widehat{\gamma})\) be a directed tree-decomposition of \(D\) of width \(w\).
	We begin by the following procedure: as long as there is a node \(x\) of \(\widehat{T}\) with no descendants and
	such that \(\widehat{\beta}(x) = \emptyset\), remove \(x\) from \(\widehat{T}\).
	Next, modify \(\widehat{T}\), by attaching below every node \(x \in V(\widehat{T})\) exactly \(\Abs{\widehat{\beta}(x)}\) children: call these
	new nodes \(\set{x_u \colon u \in \beta(t)}\).
	Let \(\widetilde{T}\) be the resulting rooted tree. Let \((\widetilde{T},\widetilde{\beta},\widetilde{\gamma})\) be a new directed tree-decomposition constructed by setting, for each $z\in V(\widetilde{T})$,
	\[\widetilde{\beta}(z) \coloneqq \begin{cases} \emptyset,& \text{ if } z \in V(\widehat{T})\text{;}\\ \set{u},& \text{ if } z = x_u\text{ for some }x\in V(\widehat{T}), u \in \widehat{\beta}(x) \text{,}\end{cases}\]
	and, for each $(y,z)\in E(\widetilde{T})$,
	\[\widetilde{\gamma}((y,z)) \coloneqq \begin{cases} \widehat{\gamma}((y,z)),& \text{ if } (y,z) \in E(\widehat{T})\text{;}\\ \set{u},& \text{ if } y\in V(\widehat{T})\textrm{ and }z = y_u\textrm{ for some } u \in \widehat{\beta}(t) \text{.}\end{cases}\]
	It is straightforward to verify that \((\widetilde{T}, \widetilde{\beta}, \widetilde{\gamma})\) is still a directed tree-decomposition of \(D\), and that the width remains unchaged.
	
	We modify \((\widetilde{T},\widetilde{\beta},\widetilde{\gamma})\) further in order to make the tree subcubic. Let \(y\) be a node of \(\widetilde{T}\)
	that has a child. (In particular, $\widetilde{\beta}(y)=\emptyset$ and $y$ is not of the form \(x_u\) for any \(x \in V(\widehat{T})\) and \(u \in \widehat{\beta}(x)\).) Let \(X \coloneqq \Gamma(y)\) (with respect to the decomposition \((\widetilde{T}, \widetilde{\beta}, \widetilde{\gamma})\)),
	and let \(d_1, \dots, d_\ell\) be an enumeration of the children of \(y\) in \(\widetilde{T}\).
	We add \(\ell\) new nodes \(p_1, p_2, \dots, p_\ell\) to our tree, with adjacency defined as follows (see \cref{fig:dtw_to_hsw}):
	\begin{itemize}
	\item \(y\) has \(p_1\) as the unique child; 
	\item for \(i < \ell\), node \(p_i\)
	has \(p_{i + 1}\) and \(d_i\) as children; and
	\item \(p_\ell\) as \(d_\ell\) as the unique child.
	\end{itemize}
	We concurrently modify \(\widetilde{\beta}\) by setting \(\widetilde{\beta}(p_i) \coloneqq \emptyset\) for each $i\in [\ell]$,
	and \(\widetilde{\gamma}\) by setting \(\widetilde{\gamma}(y p_1) \coloneqq X\), \(\widetilde{\gamma}(p_i p_{i + 1}) \coloneqq X\) for each $i\in [\ell-1]$,
	and \(\widetilde{\gamma}(p_i d_i) \coloneqq X\) for each $i\in [\ell]$.
	Let \((T, \beta, \gamma)\) be the directed tree-decomposition of $D$ obtained by applying this modification to every non-leaf node $y$ of $\widetilde{T}$. (That it is a directed tree-decomposition is easy to see.)
	\begin{figure}
		\centering
%		\includegraphics[scale=0.8]{figures/dtw_to_hsw.pdf}

		\begin{tikzpicture}
			\path[use as bounding box] (-5,-3) rectangle (5,2);
			\tikzstyle{child} = [draw,thick,isosceles triangle,rotate=90,scale=0.8]	
			\tikzstyle{help} = [draw,thick,rectangle]	
			\node (left) at (-3,0) {
				\begin{tikzpicture}
					\path[use as bounding box] (-2,-2) rectangle (2,2);
					\node[draw,thick,circle] (vertex) at (0,0) {};
					\node (parent) at ($(vertex)+(110:1.2)$) {};
					\node (parent-p) at ($(parent)+(110:0.3)$) {};
					\node[child] (child-1) at ($(vertex)+(-1.2,-1.2)$) {};
					\node[child] (child-2) at ($(vertex)+(-0.4,-1.2)$) {};
					\node[child] (child-3) at ($(vertex)+(0.4,-1.2)$) {};
					\node[child] (child-4) at ($(vertex)+(1.2,-1.2)$) {};
			
					\draw[edge] (vertex) to (child-1.east);
					\draw[edge] (vertex) to (child-2.east);
					\draw[edge] (vertex) to (child-3.east);
					\draw[edge] (vertex) to (child-4.east);
			
					\draw[edge] (vertex) to (parent);
					\draw[edge,dotted] (parent-p.center) to (parent.center);
				\end{tikzpicture}};
	
			\node (right) at (3,0) {\begin{tikzpicture}
				\path[use as bounding box] (-2,-2) rectangle (2,2);
				\node[draw,thick,circle] (vertex) at (0,0) {};
				\node (parent) at ($(vertex)+(110:1.2)$) {};
				\node (parent-p) at ($(parent)+(110:0.3)$) {};
				\node[help] (help-1) at ($(vertex)+(225:0.8)$) {};
				\node[child] (child-1) at ($(help-1)+(310:0.9)$) {};
				\node[help] (help-2) at ($(help-1)+(225:0.8)$) {};
				\node[child] (child-2) at ($(help-2)+(310:0.9)$) {};
				\node[help] (help-3) at ($(help-2)+(225:0.8)$) {};
				\node[child] (child-3) at ($(help-3)+(310:0.9)$) {};
				\node[help] (help-4) at ($(help-3)+(225:0.8)$) {};
				\node[child] (child-4) at ($(help-4)+(310:0.9)$) {};
			
				\draw[edge] (help-1) to (child-1.east);
				\draw[edge] (help-2) to (child-2.east);
				\draw[edge] (help-3) to (child-3.east);
				\draw[edge] (help-4) to (child-4.east);
			
				\draw[edge] (vertex) to (help-1);
				\draw[edge] (help-1) to (help-2);
				\draw[edge] (help-2) to (help-3);
				\draw[edge] (help-3) to (help-4);
			
				\draw[edge] (vertex) to (parent);
				\draw[edge,dotted] (parent-p.center) to (parent.center);
			\end{tikzpicture}};
	
	\node[scale=2] at ($(left)!0.45!(right)$) {\(\Rightarrow\)};
\end{tikzpicture}
		
		\caption{
			Replacing a node with multiple children by a path
			of nodes with at most $2$ children each.
		}\label{fig:dtw_to_hsw}
	\end{figure}
	
	Clearly, \(T\) is a subcubic tree and \(\{\beta(x)\colon x\in V(T)\}\) is a near partition of $V(T)$, with every non-leaf node of \(T\) assigned
	the empty set and  every leaf of \(T\) assigned a singleton set. Therefore, let $\lambda$ be the bijection mapping every leaf $x$ of $T$ to the unique vertex $u$ of $D$ such that $\beta(x)=\Set{u}$. Note that by construction, we have $|\gamma(e)|\leq w+1$ for each $e\in E(T)$. So it remains to show that $(T,\lambda,\gamma)$ is a HS-\cycledecomp of $D$ (after forgetting the orientation of the edges of $T$).
	
	To see this, consider any edge $e$ of $T$. Let $x$ be the closest ancestor of the tail of $e$ in $T$ that belongs to $V(\widetilde{T})$. By construction, we have $\gamma(e)=\Gamma(x)$. Moreover, $\lambda(\treeLower{T}{e})$ can be written as the union of a subset of $\widetilde{\beta}(x)$ and a collection of sets of the form $\widetilde{\beta}(\treeLower{\widetilde{T}}{y})$ where $y$ is a child of $x$ in $\widetilde{T}$. Since $(\widetilde{T},\widetilde{\beta},\widetilde{\gamma})$ is a directed tree-decomposition of $D$, we have that $\Gamma(x)\supseteq \widetilde{\beta}(x)$ and $\Gamma(x)$ intersects every cycle that crosses the cut $(\widetilde{\beta}(\treeLower{\widetilde{T}}{y}),\widetilde{\beta}(\treeUpper{\widetilde{T}}{y}))$, for any child $y$ of $x$. It follows that $\Gamma(x)=\gamma(e)$ intersects every cycle that crosses the cut $(\lambda(\treeLower{T}{e}),\lambda(\treeLower{T}{e}))$, so it is a valid edge-guard for $e$.
\end{proof}
%	 and \(\gamma(e)\) hits all cycles crossing the cut in \(D\)
%	induced by \(T\) and \(e\) \todo{formalise}.
%	By setting \(\lambda(t) = x\) where \(x\) is the unique element of \(\beta(t)\) when \(t\) is a leaf,
%	we obtain the desired HS-\cyclewidth decomposition of \(D\) of width at most \(w + 1\).

%\Ma{This could be neater if HS-\cyclewidth was top-minor or butterfly minor monotone, but it probably is not.}
%\Me{\cyclewidth is closed under taking butterfly minors, I would hope HS-cyclewidth is as well?}

\begin{lemma}
	\label{lem:wall_high_cyclewidth}
	Suppose \(\gridImm{3k+1}\) is a topological minor of \(D\), for some positive integer \(k\).
	Then \(D\) has HS-\cyclewidth greater than \(k\).
\end{lemma}
\begin{proof}
	%Fix a positive integer \(k\) and a digraph \(D\). 
	Let \(\ell = 3k + 1\).
	For contradiction, suppose \(D\) contains \(\gridImm{\ell}\) as a topological minor and there is a HS-\cyclewidth decomposition  \((T, \lambda, \gamma)\) of \(D\) of width at most \(k\).
	Let \(\mu\) be a minor model of \(\gridImm{\ell}\) in~\(D\).
	Let \(\CC = \set{C_1, C_2, \dots, C_{\ell}}\) be the images of the base cycles of \(\gridImm{\ell}\) under \(\mu\).
	Thus each \(C_i\) is a simple cycle in \(D\), and these simple cycles are pairwise vertex disjoint.
	Moreover, between any \(C_i\) and \(C_j\) there are \(2\ell\) pairwise vertex-disjoint paths,
	where \(\ell\) of them go from \(C_i\) to \(C_j\), and \(\ell\) of them go
	from \(C_j\) to \(C_i\) (contained within the model \(\mu\)).
	
	Consider an edge \(xy \in E(T)\).
	Its removal splits the tree \(T\) into two parts:
	\(\treeSplit{T}{x}{e}\) containing \(x\) and \(\treeSplit{T}{y}{e}\) containing $y$.
	Let \[A \coloneqq \lambda(\treeSplit{T}{x}{e}) \setminus \gamma(e)\qquad\text{and}\qquad B = \lambda(\treeSplit{T}{y}{e}) \setminus \gamma(e).\]
	Thus, \((A,B)\) is a cut of the digraph \(\gridImm{\ell} \setminus \gamma(e)\).
	In the family \(\CC\) there are at least \(\ell-k=2k+1\) cycles disjoint with \(\gamma(e)\); call those cycles \emph{surviving}.
	Since no cycle in \(\gridImm{\ell} \setminus \gamma(e)\) can contain both a vertex
	of \(A\) and a vertex of \(B\), each surviving cycle is contained entirely
	in \(A\) or entirely in \(B\). 
	
	Let us argue that in fact, all the surviving must be contained in \(A\), or all of them must be contained in~\(B\).
	Indeed, suppose $C_i,C_j\in \CC$ are surviving cycles such that \(V(C_i) \subseteq A\) and \(V(C_j) \subseteq B\).
	Since in $D$ we have \(\ell\) paths from \(C_i\) to \(C_j\) and \(\ell\) paths from
	\(C_j\) to \(C_i\), and $\ell-k=2k+1>0$, at least one of each kind avoids \(\gamma(e)\); call them \(P\)
	and \(Q\) respectively.
	We may now walk along \(P\), then along \(C_j\) till we hit the path \(Q\),
	then along \(Q\), and finally along \(C_i\) until we close a cycle; this yields
	a cycle containg a vertex of \(A\) and a vertex of \(B\), and yet avoiding \(\gamma(e)\); a contradiction.
	
	Therefore, in case that all the surviving cycles of $\CC$ are contained in \(A\), we orient the edge \(e=xy\) towards \(x\). 
	Otherwise, when all the surviving cycles are a subset of \(B\)) we orient the edge \(e\) towards \(y\).
	
	Since \(T\) is a tree, in this orientation there must be a sink.
	This sink cannot be a leaf, as each surviving cycle contains at least two vertices.
	Let \(s\) be a sink of this orientation, and let \(a, b, c\) be the edges of \(T\)
	incident to \(s\). Let \(T_a\) be the component of \(T \setminus a\)
	not containing \(s\), and similarly define \(T_b\) and \(T_c\).
	Let \[X \coloneqq \gamma(a) \cup \gamma(b) \cup \gamma(c).\]
	Set \(A \coloneqq \lambda(T_a) \setminus X\), \(B \coloneqq \lambda(T_b) \setminus X\), \(C \coloneqq \lambda(T_c) \setminus X\).
	There are at least \(\ell - 3k = 1\) cycle(s) from \(\CC\) that are disjoint with \(X\).
	By the definition of the orientation, this cycle is disjoint with each of
	\(A\),~\(B\),~\(C\), and \(X\). Yet together these \(4\) sets cover all of \(V(D)\).
	This is a contradiction.
\end{proof}

\begin{proof}[Proof of \cref{thm:cyw_dtw}]
	By \cref{lem:dtw_bounds_hsw}, we may set $\thmFkt{thm:cyw_dtw}{g}{k}\coloneqq k+1$. By \cref{thm:gridtheorem,lem:wall_high_cyclewidth}, we may set $\thmFkt{thm:cyw_dtw}{g}{k}\coloneqq 3\cdot \thmFkt{thm:gridtheorem}{g}{k}+1$.
\end{proof}
